Latency Guarantees for Caching with Delayed Hits

In the classical caching problem, when a requested page is not present in the cache (i.e., a "miss"), it is assumed to travel from the backing store into the cache "before" the next request arrives. However, in many real-life applications, such as content delivery networks, this assumption is unrealistic. The "delayed-hits" model for caching, introduced by Atre, Sherry, Wang, and Berger, accounts for the latency between a missed cache request and the corresponding arrival from the backing store. This theoretical model has two parameters: the "delay" $Z$, representing the ratio between the retrieval delay and the inter-request delay in an application, and the "cache size" $k$, as in classical caching. Classical caching corresponds to $Z=1$, whereas larger values of $Z$ model applications where retrieving missed requests is expensive. Despite the practical relevance of the delayed-hits model, its theoretical underpinnings are still poorly understood. We present the first tight theoretical guarantee for optimizing delayed-hits caching: The "Least Recently Used" algorithm, a natural, deterministic, online algorithm widely used in practice, is $O(Zk)$-competitive, meaning it incurs at most $O(Zk)$ times more latency than the (offline) optimal schedule. Our result extends to any so-called "marking" algorithm.

==> sections/0_abstract.tex <==
In the classical caching problem, when a requested page is not present in the cache (i.e., a ``miss''), it is assumed to travel from the backing store into the cache \emph{before} the next request arrives. However, in many real-life applications, such as content delivery networks, this assumption is unrealistic.

The \emph{delayed-hits} model for caching, introduced by Atre, Sherry, Wang, and Berger, accounts for the latency between a missed cache request and the corresponding arrival from the backing store. This theoretical model has two parameters: the \emph{delay} $Z$, representing the ratio between the retrieval delay and the inter-request delay in an application, and the \emph{cache size} $k$, as in classical caching. Classical caching corresponds to $Z=1$, whereas larger values of $Z$ model applications where retrieving missed requests is expensive. Despite the practical relevance of the delayed-hits model, its theoretical underpinnings are still poorly understood.

We present the first tight theoretical guarantee for optimizing delayed-hits caching: The ``Least Recently Used'' algorithm, a natural, deterministic, online algorithm widely used in practice, is $O(Zk)$-competitive, meaning it incurs at most $O(Zk)$ times more latency than the (offline) optimal schedule. Our result extends to any so-called ``marking'' algorithm.


==> sections/4_z-2_upper_bound.tex <==

\section{Upper bound at delay $2$}\label{sec:z=2}


We now turn our attention to the setting in which $Z \in O(1)$. By definition, $Z=1$ corresponds to the traditional offline caching problem, solved optimally through B\'el\'ady's rule. This section is devoted to extending tractability to $Z = 2$, thereby establishing \Cref{thm:z=2}.

The basis of our proof is reducing $\twocache$ to a problem we call $\kwtcache$. $\kwtcache$ has no concept of ``delay'' in serving requests, so there are no $\sDHit$s; however, every request comes with a \emph{weight} $w_t$, and the latency penalty is $w_t$ if the request is missed.\footnote{$\kwtcache$ is a variant of weighted caching problems which have appeared in the literature. In particular, Chrobak, Karloof, Payne, and Vishwanathan~\cite{CKPV91} analyze a special case of our problem where every time a page is requested, it is requested with the same weight.} We define the finite state machine formally for \Cref{fig:fsm:weighted-caching}.

\input{figures/fsm_server}

\input{figures/fsm_weighted_caching}


\begin{theorem}
    For all $k,n$, there is an $O(kn^2)$-time algorithm for $\kwtcache$.
\end{theorem}

\begin{proof}[Proof sketch]
    The proof is a simple modification of the reduction by Chrobak, Karloof, Payne, and Vishwanathan~\cite{CKPV91} from their weighted caching variant to the standard $\kserver$ problem. This construction consists of building a finite metric space $M_\rseq = (X, d)$ whose optimal solution for the $k$-server problem has the same cost as the optimal caching policy, with cache size $k$, over $\rseq$. Concretely, if $T = |\rseq|$, then $X = [T] \times [n]$. We view $X$ as partitioned into $T$ \emph{layers} $L_t = \{t\} \times [n]$, each a copy of $[n]$. The $n$ vertices in the layer $L_i$ correspond to the $n$ pages a policy could potentially have on its cache at time $t$, and the locations of the $k$ servers at time $t$ by any $k$-server policy $A$ will determine exactly which pages are on the cache of its associated caching policy $A'$.
    
    For each pair of vertices $(t,a) \neq (s,b) \in X$ where $t \leq s$, we define a \emph{directed} edge weight
    \[
    e((t,a),(s,b)) = \begin{cases}
        0 & \text{if } t < s \text{ and } a = b\\
        w_s & \text{if } t < s \text{ and } a \neq b\\
        \infty & \text{otherwise.}
    \end{cases}
    \]
    Note that these weights are in fact a metric.
\end{proof}

\begin{proof}[Proof of \Cref{thm:z=2}]
    In $\twocache$ pages are unweighted. To convert an instance of $\twocache$ to an instance of $\kwtcache$, we use \emph{artificial} weights to model the impact of latency. In particular, suppose the input $\rseq$ to $\twocache$ is divided into maximal runs of consecutive pages. For example, 
    \[
    \rseq = 1,2,3,3,3,2,1,1,2 \quad \to \quad 1 \mid 2 \mid 3,3,3 \mid 2 \mid 1,1 \mid 2.
    \]
    Now, the key insight is that runs of length $1$ behave exactly the same as in the $Z=1$ case, but incur penalty $2$ in the case of a $\sMiss$, whereas runs of length $r > 1$ incur in cost $3$ regardless of $r$. Thus, we can \emph{compress} the delayed hits request sequence into a weighted caching request sequence, by transforming isolated requests for a page $p$ into weight-$2$ requests and runs (of length $> 1$) of requests for $p$ into weight-$3$ requests.
\end{proof}

==> sections/99_OLD_INTRO.tex <==

In this paper, we present some theoretical results on policies for a problem called \emph{delayed hits caching}, as well as simulations of these and other policies. We begin by presenting background for this problem, and then present our results.

\subsection{Background and motivation}

\emph{Caching} is a landmark problem in computer science of immense relevance in computer systems and other applied areas. The basic motivation for caching is to help service requests for chunks of stored data, typically called \emph{pages}, which may be very slow. The fundamental insight of caching is \emph{locality}: Some pages may be requested much more frequently than others, especially on short timescales. Thus, it may make sense to maintain a \emph{cache} of a small number of pages, such that requests for these pages can be served instantaneously, without having to wait for the data to be retrieved from the underlying storage medium.

\begin{table}
    \small \centering
    \begin{tabular}{c|c|c}
        \textbf{Application} & \textbf{Main store} & \textbf{Cache} \\ \hline
        Memory & Main (e.g., DRAM) & In-CPU (e.g., DRAM) \\
        File storage & Hard drive & Main memory \\
        Web content & Faraway CDN servers & Nearby ``edge`` servers \\
    \end{tabular}
    \caption{Some basic applications of caching in computer systems.}
\end{table}

In the simplest model of caching, when a new request arrives for a page $p$, one of two things happens:

\begin{enumerate}
    \item A \emph{cache hit}: $p$ is already present in the cache. We can serve the request for $p$ instantaneously.
    \item A \emph{cache miss} (or \emph{page fault}): $p$ is absent from the cache. We must ``fetch'' $p$ from the underlying storage medium, incurring a latency penalty, and also choose which page to \emph{evict} from the current cache in order to make room for $p$. The choice of which page to evict is determined by a \emph{caching policy}.
\end{enumerate}

In the history of computer systems, many early cache designs were \emph{blocking}: After a cache miss, the entire system would ``freeze'', serving no more requests, until the missed request was served from the backing store. Pioneering works such as \cite{Kro81} in the area of processor design proposed \emph{non-blocking caches}: In the period immediately after a miss, the cache could continue serving hits, and it would ``circle back'' with responses to missed hits when these responses became available from the backing store. This introduces a third possibility for what happens when a page $p$ is requested: $p$ is not present in the cache, but it is already \emph{in transit} from the backing store. This possibility is called a \emph{delayed hit}, and the latency it incurs is intermediate between that of a hit and a miss. See \Cref{fig:dhits-ex} below for an example. We refer to the line of pages in transit from the store to the cache as the \emph{queue}.

Applications in recent years have had unfettered growth in throughput demands, leading to an increased lag in the number of requests arriving during a fetch. Atre \emph{et al.}~\cite{ASWB20} argue that as the ratio \[ Z = \frac{\text{inter-request time}}{\text{cache miss latency}} \] increases, the consideration of delayed hits has become increasingly important. When fetching lag is short, i.e., $Z$ is small, a cache miss can be served within the time before the next request is received --- the model degenerates into traditional caching without delayed hits. Even when $Z$ is still small, the problem still may resemble traditional caching and traditional caching wisdom may still apply (though there is a lack of formal results to this effect).

The importance of considering delayed hits arises in any setting where latencies greatly exceed throughputs. For instance, statistical models of delayed hits were studied in works including \cite{TRTD98,GE08}, which studied the difference between L1 and L2 cache latencies within a processor and showed that modeling delayed hits enables significant improvements in predicting overall cache performance. While these works did not study the $Z$ ratio explicitly, they suggest that $Z$ is sufficiently large in the setting of processor caches that the effects of delayed hits become salient.

According to \cite{ASWB20}, there is a broad trend of increasing $Z$ across many computer systems contexts caused by increasing request throughputs without concomitant decreases in latencies. Indeed, latencies may already be near-minimal in some settings given underlying physical limitations, e.g., spatial distances between the request handler and the backing store. For instance, Katz-Bassett \emph{et al.}~\cite{KJK+06} show that in 2006, end-to-end round-trip latencies on the global Internet were already less than $3$ times slower than the fastest possible round-trip latencies given by the speed of light.  In the setting of \emph{content distribution networks (CDNs)}, missing a request at the proxy server near to a client may trigger a request to a faraway central server incurring such large latencies. \cite{ASWB20} estimates that $Z$ in this case is on the order of $200\, 000$. Delayed hits in the context of CDNs were also studied by Zhang \emph{et al.}~\cite{ZTL+22}. \cite{ASWB20} also cites the authors' own implementation of an FPGA software switch, where they measured that local SRAM reads took only $5$ ns while, after misses, the required DRAM reads took $100$ ns (a factor $Z=20$ difference).

The impact of delayed hits in high-$Z$ caching environments motivates the design of a theoretical model of delayed hits, undertaken by Atre \emph{et al.}~\cite{ASWB20}, and investigations, including our own, into when caching can perform well even in the presence of delayed hits. 

\begin{figure*}
    \centering
    \begin{tikzpicture}[scale=0.5]
    \fill[blue, opacity=0.2] (2+2+2, -2) -- (2+2+2, 4) -- (5+2+2, 4) -- (5+2+2, -2) -- (2+2+2, -2);

    \onesquare{0.0+2}{2.0}{gray!20!white}{1};
    \onesquare{0.0+2}{1.0}{gray!20!white}{2};
    \onesquare{0.0+2}{0.0}{gray!20!white}{4};

    \draw[->, thick] (4+2, 1) -- (0.5+2,1);
    \node (z) at (2.25+2, 0.5) {$Z = 10$};
    \node (cache) at (0+2, 4) {$\textsc{Cache}$};
    \node (k) at (0+2, 3.25) {$k = 3$};
    \node (st) at (5.5+2, 1) {$\textsc{Store}$};

    \onesquare{5.5+2}{3}{gray!20!white}{3};
    \onesquare{5.5+2}{2}{gray!20!white}{5};
    \onesquare{5.5+2}{0.0}{gray!20!white}{6};
    \onesquare{5.5+2}{-1}{gray!20!white}{7};

    \node (sigma) at (-7.5, 2.5) {$\textsc{Request Sequence } \rseq $ };
    \newcommand{\lambdaDist}{1.5}
    \onesquare{-2*\lambdaDist}{1.0}{red!50!white}{3};
    \onesquare{-3*\lambdaDist}{1.0}{green!50!white}{1};
    \onesquare{-4*\lambdaDist}{1.0}{red!20!white}{3};
    \onesquare{-5*\lambdaDist}{1.0}{green!50!white}{2};
    \onesquare{-6*\lambdaDist}{1.0}{green!50!white}{4};
    \onesquare{-7*\lambdaDist}{1.0}{green!50!white}{1};
    \onesquare{-8*\lambdaDist}{1.0}{red!50!white}{5};
    \onesquare{-9*\lambdaDist}{1.0}{green!50!white}{2};

    \foreach \i in {1,...,8}{
        \node (\i) at (-1.5 - \lambdaDist*\i, 1.75) {\tiny $\i$};
    }

    
    \draw [
    thick,
    decoration={
        brace,
        mirror,
        raise=0.5cm
    },
    decorate
] (-4, 1.4) -- (-3.5,1.4);

\node (lambda) at (-3.75, -0.2) {$\lambda$};

\draw[-, dashed, thick, red] (-2+2, -3) -- (8+2, -3) -- (8+2, 5) -- (-2+2, 5) -- (-2+2, -3);

\node[color=red!80!black] (system) at (5, 6) {$\textsc{System}$};
    
    \end{tikzpicture}
    \caption{Illustration of a caching system in the delayed hits model. The time of each request is displayed above it, and the color of each request represents its associated penalty; cache hits are colored in green, cache misses are colored in opaque red and delayed hits are colored in pale red. The cache starts out containing $1,2,4$. With a delay of $Z=10$, page $3$, requested at the first time step, does not arrive until the entire sequence completes, incurring a latency of $10$. The first missed request for $3$ is followed two time steps later by another request for $3$; this incurs a latency of only $8$, since page $3$ will arrive in only $8$ more steps. Finally, the request for page $5$ at time step $7$ is also a miss, incurring a latency of $10$. The total latency is therefore $28$.}
    \label{fig:dhits-ex}
\end{figure*}

\subsection{Results}

In this section, we highlight the major results of our paper. See the following section (\Cref{sec:model}) for formal definitions of the terms used.

\begin{theorem}\label{thm:lru-bound}
    If $Z < k \in \mathbb{N}$, the ``least recently used'' policy $\PLRU$ achieves competitive ratio $O(kZ)$ for $\Zkdhits$ on streams.\footnote{Technical note: For now, we only know how to prove this for request sequences containing at least $\Omega(1)$ \emph{phases}, though this is not an unrealistic assumption; see the proof for details.}
\end{theorem}

\Cref{thm:lru-bound} is proven in \Cref{sec:lru-bound} below. Its analysis is a more complicated variant on the standard analysis of LRU in the traditional caching model, which shows that in that model, LRU achieves competitive ratio $O(k)$. We remark that one basic reason that the $Z<k$ assumption is helpful is that it guarantees when a page $p$ is arriving off the queue, it has been used more recently than at least one page in the cache, since there are $k$ pages in the cache, while $p$ was requested at most $Z$ steps ago, and so LRU never wants to evict a page which has just arrived off the queue.

\begin{theorem}\label{thm:z=2}
For all $k$, the $(2,k)$-\dhits~problem  can be solved in polynomial time.
\end{theorem}

\Cref{thm:z=2} is proven in \Cref{sec:z=2} below. Briefly, the proof shows that in the $Z=2$ case, $\Zkdhits$ reduces to a \emph{weighted} caching problem, where polynomial-time algorithms are already known.

\subsection{Related work}

The theoretical study of caching was initiated by B\'el\'ady in 1966~\cite{belady}. A key contribution of his work, now known as \emph{B\'el\'ady's rule}, was an optimal \emph{offline} policy for caching: At each time step, evict whichever page is requested the \emph{furthest-in-the-future} (FIF). Given that B\'el\'ady's rule assumes knowledge of the future requests, a great deal of work then centered around the question of whether similar performance to the FIF policy could be achieved by an \emph{online} policy, that is, a policy that, at each time step, chooses a page to evict only using knowledge of \emph{past} requests. This line of research resulted in a wide variety of online caching policies (e.g., \emph{least recently used} (LRU) and \emph{first-in-first-out} (FIFO)), which were analyzed through the incipient-at-the-time lens of~\emph{competitive analysis}, which compares the latencies achieved by online and offline algorithms~\cite{sleator}. Shortly afterwards, many optimal online policies for caching were fully understood~\cite{Fiat_1991}, both in deterministic and randomized settings. 

Since then, attention has shifted towards challenging some of the assumptions of the basis caching model. For example, more complex models allow pages to have heterogeneous sizes (affecting how many pages can be placed in the cache simultaneously) and costs (affecting the penalty incurred to fetch a missing page)~\cite{irani}. Other works question the assumption that fetched pages enter the cache immediately after a page fault (i.e., before the next request arrives). In other words, the traditional model assumes that the average fetching time $Z$ of a page going from the underlying memory store to the cache is smaller than the average time between requests $\lambda$. The work of Atre \emph{et al.}~\cite{ASWB20} introduced the \emph{delayed hits model}, in which the fetching time $Z$ is non-negligible, and thus a page $p$ requested $t < Z$ units of time after a page fault will require more time to be served than a \emph{hit} but less time than a page fault, thus constituting a \emph{delayed hit}. This model is particularly applicable to the context of CDNs in which the time between requests is much smaller than the time to fetch objects to the cache.

Atre \emph{et al.}\ proved that B\'el\'ady's rule is not an optimal (offline) policy for caching with delayed hits, and presented both integer linear programming (ILP) and minimum-cost multi-commodity flow (MCMCF) formulations for the problem of finding an optimal offline policy given a request sequence. As both the ILP and the MCMF problems are NP-hard in general, a tantalizing open question is whether the offline optimal policy for caching with delayed hits can be computed in polynomial time or if it is NP-hard.\footnote{In terms of complexity analysis of caching problems, a long-standing open problem was proving strong hardness for general caching (i.e., with page costs and/or sizes)~\cite{albers}, solved by the break-through result of Chrobak \emph{et al.}~\cite{chrobakCachingHardEven2010}~in 2010, and then refined (e.g., to page sizes in $\{1,2,3\}$) in a series of work~\cite{DARMANN20104217, folwarcznyGeneralCachingHard2017,bonsma}.}

In follow-ups to the work of Atre \emph{et al.}, Manohar and Williams~\cite{MW20} studied policies for caching with delayed hits. They proved a lower bound on the competitive ratio of deterministic online policies, and also constructed situations where the delayed hits model of Atre \emph{et al.} displayed counterintuitive ``non-antimonotone'' behavior. Carleton \emph{et al.}~\cite{Car21a} empirically simulated an extension of the delayed-hits model to multiple tiers of caching and evaluated the performance of some simple heuristics. Yan and Li~\cite{YL22} studied a setting where requests may have very heterogeneous demands, and showed that a simple heuristic policy is optimal if the input is stochastic (a Poisson process). Zhang \emph{et al.}~\cite{ZTL+22} added a ``bypassing'' option to the model, where requests can be served directly by the remote server without the result also being stored in the cache, and analyzed an online policy in this setting.
